Nonabelian Fourier Kernels on $\mathrm{SL}_2$ and $\mathrm{GL}_2$

For $G=\mathrm{SL}_2$ or $\mathrm{GL}_2$, we present explicit formulas for the nonabelian Fourier kernels on $G$, as conjectured by A. Braverman and D. Kazhdan. Additionally, we furnish explicit formulas for the orbital Hankel transform on $G$, a topic investigated by the second author, and provide an explicit formula for the stable orbital integral of the basic function. These results are applicable to local fields with residual characteristics other than two.

==> Cp_7_Kernel.tex <==

% !TEX root = luo-ngo.tex

\section{Some explicit formulas related to the nonabelian Fourier kernel}\label{sec:FKsl2gl2}

In this section, we discuss explicit formulas for the nonabelian Fourier kernels for $G=\SL_2$ or $\GL_2$. We also discuss the constructions of the nonabelian $\rho$-Fourier kernels proposed as plausible by the second author and Lafforgue. Although these constructions fail to give the correct answer for general symmetric powers $\rho$, they lead to the correct construction presented in this article.

\subsection{An explicit formula}\label{subsec:aformulaFK}

Fix a finite dimensional representation $\rho:\LG\to \GL(V_\rho)$. By Conjecture \ref{conjec:bknproposal}, our goal is to construct a (stably) invariant distribution $\RJ^\rho_\psi$, such that after regularization, the action of $\RJ^\rho_\psi$ on any irreducible admissible representation $\pi$ of $G(F)$ is equal to the scaling action by the Langlands local gamma function $\gam(-\frac{n_\rho-1}{2},\pi^\vee,\rho,\psi)$. Not surprisingly, Theorem \ref{thm:descentheuristic:sl2}, Theorem \ref{thm:descentheuristic:gl2} and Theorem \ref{thm:inv} provides the desired explicit construction for the nonabelian Fourier kernel $\RJ^{\rho}_\psi$ based on datum on tori $\{\RJ^{\rho}_{\psi,T}\}$, where $T$ runs over stable conjugacy classes of maximal tori in $G$. Notice that after multiplying a smooth and compactly supported function on the determinant factor, we can assume that $\{\RJ^\rho_{\psi,T}\}$ actually lies in the Bernstein center of $T(F)$ (and its archimedean variant, which are given by invariant tempered distributions that are of moderate growth on the tempered dual of $T(F)$). 

Starting from the nonabelian Fourier kernel $\RJ^{\rho}_{\psi}$ on $G(F)$, for any dihedral representation $\CW_\chi$ of $G(F)$ attached to a character $\chi:E^\times \to \BC^\times$, from Theorem \ref{thm:descentheuristic:gl2}, the left hand side of Theorem \ref{thm:descentheuristic:gl2} will provides the constant
$$
\gam(-\frac{n_\rho-1}{2},(\CW_\chi)^\vee,\rho,\psi).
$$
Now by \cite{gl2llc}, under local Langlands correspondence for $\GL_2$, the local $L$-parameter for $\CW_\chi^\vee$ is given by $(\Ind_{W_E}^{W_F}\chi)^\vee\simeq \Ind_{W_E}^{W_F}\chi^{-1}$, 

Without loss of generality, let us for convenience assume that $G=\GL_2$ and $\rho=\Sym^n$. Since $\LG = \GL_2(\BC)$, up to direct sum and twist by determinant, by explicit calculation or \cite[Thm.~1.0.2]{DanielZhilin}, $\rho\circ \Ind^{W_F}_{W_E}\chi^{-1}$ is a direct sum of one dimensional character or two dimensional dihedral representations attached to $E$ and the induced character depends only on $\chi$. The description is uniform over local field of odd residual characteristic. In particular, from \cite[Thm.~4.7]{jlgl2}, 
$$
\gam(s,\Ind^{W_F}_{W_E}\chi,\psi_F) = 
\gam(s,\chi,\psi_E)\cdot \lam_{E/F}.
$$
It follows from the decomposition of local $L$-parameters as in \cite[Thm.~1.0.2]{DanielZhilin} that there exists a constant $\kappa^{\rho}_{E/F}= \lam_{E/F}^{\ceil{\frac{n-1}{2}-1}}$ depending only on the quadratic extension $E/F$, $\rho$ and $\psi$ only, such that 
\begin{equation}\label{eq:nonabfourier:gl2:1}
\gam(-\frac{n_\rho-1}{2},(\CW_\chi)^\vee,\rho,\psi) = 
\gam(-\frac{n_\rho-1}{2},\chi^{-1},\rho,\psi_E)\cdot 
\kappa^\rho_{E/F}
\end{equation}
where $\rho$ on the right hand side is the restriction to the dual group of the torus attached to $E^\times$. Now following Theorem \ref{thm:descentheuristic:gl2}, the right hand side of \eqref{eq:nonabfourier:gl2:1}, after regularization, should be equal to the the Mellin transform of a distribution on the torus $E^\times$. But such a distribution has already been constructed in subsection \ref{subsec:toruscase} which is actually a smooth function on the maximal torus. To make it precise, for any étale quadratic $F$-algebra $E$, the discussion in subsection \ref{subsec:toruscase} provides a smooth function $\RJ^{\rho}_{\psi,T_E}$ such that for any character $\chi_s = \chi|\det_{T_E}|^s$ of $T_E(F)$ where $T_E$ is a maximal torus determined by $E$, after regularization, 
$
\chi_s(\RJ^\rho_{\psi,T_E}) = \gam(-s,\chi^{-1},\rho,\psi).
$
As a corollary, the following identity holds for the Mellin transform of $\kappa^{\rho}_{E/F}|\Nr_{E/F}(\cdot)|^{\frac{n_\rho+1}{2}}\RJ^\rho_{\psi,E}$ evaluated at $\chi$:
$$
\chi(\kappa^{\rho}_{E/F}|\Nr_{E/F}(\cdot)|^{\frac{n_\rho+1}{2}}\RJ^\rho_{\psi,T_E}) = \gam(-\frac{n_\rho-1}{2},\chi^{-1},\rho,\psi_E)\kappa^\rho_{E/F} = 
\gam(-\frac{n_{\rho}-1}{2},(\CW_\chi)^{-1},\rho,\psi).
$$
Comparing with the descent formula in Theorem \ref{thm:descentheuristic:gl2}, we set, for any étale quadratic $F$-algebra $E$, the following functions 
\begin{align}\label{eq:desentdatum:FKgl2}
\big\{\RJ_E = \kappa^\rho_{E/F}
|\Nr_{E/F}(\cdot)|^{\frac{n_\rho}{2}+1}
\RJ^\rho_{\psi,T_E}\big\}_{E/F}.
\end{align}
Then Theorem \ref{thm:inv} provides us with a function $\RJ^{\rho,\p}_{\psi}$ on $\Fc_G(F)$, which, over the split locus, is equal to $|\Nr_{F\oplus F/F}(\cdot)|^{\frac{n_\rho}{2}+1}\RJ^\rho_{\psi,F\oplus F}$, such that the following descent formula holds
$$
\lam_{E/F}\CG\CG_E(\RJ^{\rho,\p}_\psi)\big(
\Tr(e),\Nr(e)
\big) = 
\kappa^\rho_{E/F}
\RJ^{\rho}_{\psi,E}
\big(
\Tr(e),\Nr(e)
\big)
|\Nr(e)|^{\frac{n_\rho}{2}+1},\quad e\in E^\times.
$$
Now based on Definition \ref{defin:aux:sl2}, we can set 
$$
\RJ^{\rho}_{\psi} := \mathrm{Laf}(\RJ^{\rho,\p}_\psi).
$$
Then following the discussion in section \ref{sec:descent} and section \ref{sec:inv}, for any dihedral representation $\pi_{\chi_E}$ attached to a character $\chi:E^\times \to \BC^\times$ of an étale quadratic $F$-algebra $E$, 
$$
\pi_{\chi_E}(\RJ^\rho_\psi) = 
\kappa^\rho_{E/F}
\gam(-\frac{n_\rho-1}{2},\chi^{-1},\rho,\psi_E) = 
\gam(-\frac{n_\rho-1}{2},(\CW_\chi)^\vee,\rho,\psi).
$$
Hence $\RJ^\rho_\psi$ is the desired $\rho$-Fourier kernel. In conclusion we derive an explicit formula for $\RJ^\rho_\psi$ from $\{\RJ^\rho_{\psi,E}\}_{E/F}$ based on the inversion theorem \ref{thm:inv}.




\subsection{Low symmetric power examples}\label{subsec:excepex}

In \cite{ngo2016hankel}, the second author shows that the distributions $\{\RJ^\rho_{\psi,T}\}_{T\subset G}$ can be patched together directly to get a stable function on $\Fc_{G}(F) = (G\sslash \Ad(G))(F)$, which we denote as $\RJ^\rho_{\psi,\mathrm{Ngo}}$. Later, when $G=\SL_2$ or $\GL_2$, Lafforgue (\cite{lafforguegl2}) suggests that modulo the convergence, one need to apply the Lafforgue transform as in Definition \ref{defin:aux:sl2} to get the correct distribution, which we denote as $\RJ^\rho_{\psi,\mathrm{Laf}}:= \mathrm{Laf}(\RJ^\rho_{\psi,\mathrm{Ngo}})$. In the following, we discuss three examples related to their constructions.


\subsubsection{$G=\GL_2,\rho=\std$}

When $G=\GL_2$ and $\rho=\std$. This is the case considered by Godement and Jacquet (\cite{gjzeta}). In this case, $\RJ^{\rho}_\psi(\tr(g)) = \psi(\tr(g))$ and $\RJ^{\rho}_{\psi,E}(\tr(e)) = \psi(\tr(e))$ are the standard Fourier kernels. Therefore $\RJ^{\rho}_{\psi,\mathrm{Ngo}}  =\RJ^{\rho}_{\psi}$. On other other hand, since the Fourier inversion of $\RJ^{\rho}_{\psi}$, denoted as $\wh{\RJ}^{\rho}_{\psi} = \CF_{\psi^{-1}}(\RJ^\rho_\psi)$, is given by the delta mass supported at $\xi=1$, $\RJ^{\rho}_{\psi,\mathrm{Laf}} = \RJ^{\rho}_{\psi,\mathrm{Ngo}} = \RJ^{\rho}_{\psi}$ and the constructions of Lafforgue and the second author work for this situation.


\subsubsection{$G=\BG_m\times \SL_2,\rho=\Sym^2$}

Now let us look at the case when $G=\BG_m\times \SL_2$ and $\rho=\Sym^2$, i.e. $\LG = \BC^\times\times \SO_3(\BC)$ and $\rho$ is the standard embedding of $\SO_3$ into $\GL_3$, together with the central scaling action of $\BG_m$. This is the case considered in \cite{JLZ} (based on \cite{doubling}) over a $p$-adic field. In this case, as shown in \cite{JLZ}, for $(a,g)\in F^\times \times \SL_2(F)$, 
$$
\RJ^{\rho}_{\psi}(a,\tr(g)) = \eta_\psi(2a+\tr(g))
$$
where $\eta_{\psi}$ is a smooth function on $F^\times$ with the property that for any character $\chi$ of $F^\times$, the following regularized Mellin transform holds as a meromorphic function of $s\in \BC$,
$$
\int^\pv_{F^\times}
\chi^{-1}(x)|x|^{-s}\eta_\psi(x)\ud^*x = 
\gam(s+1,\chi,\psi)\gam(s+2,\chi^2,\psi)
$$
where $\gam(s,\chi,\psi)$ is the local Tate gamma factor (\cite{tatethesis}). For the definition of the regularization, see \cite{JLZ} for details. Formally, we can also write $\RJ^\rho_\psi$ as follows,
$$
\RJ^\rho_{\psi}(a,\tr(g)) = 
\int^\pv_{F^\times}
\psi(z+\frac{2a+\tr(g)}{z^2})|z|^{-2}\ud^*z.
$$
The intgral on the right hand side is not absolutely convergent and regularization is also needed.

In the following, let us compute $\RJ^\rho_{\psi,\mathrm{Ngo}}$ and $\RJ^{\rho}_{\psi,\mathrm{Laf}}$ and compare them with $\RJ^\rho_\psi$. 

We first compute $\RJ^\rho_{\psi,\mathrm{Ngo}}$. We follow the presentation in subsection \ref{subsec:toruscase}. The restriction of $\rho$ to the diagonal split torus of $\BG_m\times \SO_3$ is given by $(a,\diag(t,1,t^{-1}))\mapsto \diag(at,a,at^{-1})\in (\BG_m)^3\subset \GL_3$. Passing to the dual side, we get the following homomorphisms
\begin{num}
    \item 
    For any étale quadratic $F$-algebra $E$, let $T_E = \BG_m\times \ker(\Nr_{E/F}:\Res_{E/F}\BG_m\to \BG_m)$ be the maximal torus of $\BG_m\times \SL_2$ determined by $E$, then 
\begin{align*}
\rho_E: \BG_m\times \Res_{E/F}\BG_m&\to \BG_m \times \ker(\Nr_{E/F}:\Res_{E/F}\BG_m\to \BG_m)
\\
(x_2,y)&\mapsto (x_2\Nr_{E/F}(y),\frac{y}{\iota(y)}).
\end{align*}
where $\iota$ is the unique nontrivial involution attached to $E/F$.
\end{num}
For any étale quadratic $F$-algebra $E$, the kernel of $\rho_E$ is always isomorphic to $\BG_m$. Passing to $F$-points, for $(a,e)\in F^\times \times E^1$, we are pushing forward $\psi(x_2+\tr_{E/F}(y))$ along the fiber 
$$
x_2\Nr_{E/F}(y) = a, \frac{y}{\iota(y)} = e,\quad x_2\in F^\times, y\in E^\times.
$$
Choose a representative $y_e\in E^\times$ such that $y_e(\iota(y_e))^{-1} = e$. Then we are pushing forward $\psi(x_2+z\tr_{E/F}(y_e))$ along the fiber
$$
x_2\Nr_{E/F}(y_e)z^2 = a,\quad x_2,z\in F^\times.
$$
Equivalently, we are integrating $\psi(\frac{a}{z^2\Nr_{E/F}(y_e)}+z\tr_{E/F}(y_e))$ along $z\in F^\times$. Changing variable $z\mapsto \frac{z}{\tr_{E/F}(y_e)}$, we get 
$$
\RJ^\rho_{\psi,\mathrm{Ngo}}(a,\tr(e)) = 
\int^\pv_{z\in F^\times}
\psi\bigg(
\frac{a}{\frac{z^2\Nr_{E/F}(y_e)}{\tr_{E/F}(y_e)^2}}
+
z
\bigg)
\ud^*z
=
\int^\pv_{z\in F^\times}
\psi
(
\frac{2a+\tr(e)}{z^2}+z
)
\ud^*z.
$$
Equivalently, 
$$
\RJ^\rho_{\psi,\mathrm{Ngo}}(a,\tr(g)) = 
\wt{\eta}_\psi(2a+\tr(g))
$$
with 
$$
\int^\pv_{F^\times}
\chi^{-1}(x)|x|^{-s}\wt{\eta}_\psi(x)\ud^*x = 
\gam(s+1,\chi,\psi)\gam(s+1,\chi^2,\psi).
$$
In particular, $\RJ^{\rho}_{\psi,\mathrm{Ngo}}\neq \RJ^\rho_\psi$. It turns out that as speculated in \cite{lafforguegl2}, the Lafforgue transform $\RJ^\rho_{\psi,\mathrm{Laf}}:= \mathrm{Laf}(\RJ^\rho_{\psi,\mathrm{Ngo}})$ remedies the discrepency between $\RJ^\rho_{\psi}$ and $\RJ^\rho_{\psi,\mathrm{Ngo}}$. To make it precise, by direct calculation, 
\begin{equation}\label{eq:exceptionaleg:1}
\wh{\RJ}^{\rho}_{\psi,\mathrm{Ngo}}(a,\xi):=
\CF_{\psi^{-1}}({\RJ}^{\rho}_{\psi,\mathrm{Ngo}})(a,\xi) = 
\psi(2a\xi)
\CF_{\psi^{-1}}(\wt{\eta}_\psi)(\xi)
=
\psi(2a\xi)
\int_{z^2\xi=1}
\psi(z)\ud^*z
\end{equation}
and therefore by carefully analyzing the convergence involved,
$$
\RJ^\rho_{\psi,\mathrm{Laf}}(a,\tr(g)) := 
\int_{\xi\in F}
\psi(\xi \tr(g))
|\xi|
\wh{\RJ}^\rho_{\psi,\mathrm{Ngo}}(a,\xi)\ud \xi
=
\int_{z\in F^\times}^\pv
\psi(z+\frac{2a+\tr(g)}{z^2})|z|^{-2}\ud^*z
$$
which is exactly equal to $\RJ^\rho_{\psi}(a,\tr(g))$.

\begin{rmk}\label{rmk:exceptionaleg}
Unfortunately the remedy of Lafforgue still fails in general, which will be shown in the next example. Before preceding, let us explain why the construction of Lafforgue works for $G=\BG_m\times \SL_2$ and $\rho=\Sym^2$ intuitively. From \eqref{eq:exceptionaleg:1}, the functions $\wh{\RJ}^{\rho}_{\psi,\mathrm{Ngo}}$ and $\wh{\RJ}^{\rho}_\psi$ are supported on $(F^\times)^2$. In particular, since the quadratic character $\eta_E$ is trivial on $(F^\times)^2$ for any quadratic extension $E/F$, the descent formula in Theorem \ref{thm:descentheuristic:sl2}, when applied to $\RJ^{\rho}_\psi$, can be reduced to 
$$
\CD_E(\RJ^\rho_\psi)(\Tr(e)) = \mathrm{Laf}(\RJ^{\rho}_{\psi})(\Tr(e)),\quad e\in E^1.
$$
Moreover, from \cite[Thm.~4.7]{jlgl2}, $\gam(s,\Ind^{W_F}_{W_E}\chi,\psi_F) = \gam(s,\chi,\psi_E)\cdot \lam_{E/F}$. Hence one can deduce that 
$$
\mathrm{Laf}(\RJ^{\rho}_{\psi}) = 
\RJ^{\rho}_{\psi,\mathrm{Ngo}}.
$$
In conclusion, the remedy of Lafforgue crucially relies on the fact that the trace variable of $\wh{\RJ}^{\rho}_{\psi}$ is supported on $(F^\times)^2$, and the difference between the local gamma factors on $G(F)$ and $F^\times \times E^1$ is given by $\lam_{E/F}$. However, in general there do exist  nonabelian Fourier kernels (which is shown in the next example) whose Fourier inversion in trace variable are not supported on $(F^\times)^2$, and the discrepancy between the local gamma factors on $G(F)$ and $E^1$ differs more than just the constant $\lam_{E/F}$ as shown in previous subsection. Hence a more sophisticated inversion formula is needed. 
\end{rmk}


\subsubsection{$G=\GL_2\times_{\det} \GL_2,\rho = \otimes$}

Finally let us look at the case when $G=\GL_2\times_{\det}\GL_2 = \{(g_1,g_2)\in \GL_2\times \GL_2\mid \det g_1=\det g_2\}$ and $\rho=\otimes$. The integral representation for the corresponding $L$-functions can be obtained via a slight variant of doubling method (\cite{doubling}). In particular, following the same argument as \cite{JLZ}, one can show that the distribution $\RJ^\rho_{\psi}$ is given as follows
$$
\RJ^\rho_{\psi}(\det,\tr(g_1),\tr(g_2)) = 
\wb{\eta}_\psi(\tr(g_1)+\tr(g_2))
$$
with $\wb{\eta}_\psi$ a smooth function on $F^\times$ whose regularized Mellin transform gives
$$
\int^\pv_{F^\times}
\chi^{-1}(x)|x|^{-s}
\wb{\eta}_\psi(x)\ud^*x = 
\gam(s+1,\chi,\psi)\gam(s+3,\chi,\psi).
$$
We can also write $\RJ^\rho_{\psi}$ as follows
$$
\RJ^\rho_{\psi}(a,\tr(g_1),\tr(g_2)) = 
\int^\pv_{F^\times}\psi(z+\frac{\tr(g_1)+\tr(g_2)}{z})
|z|^{-2}\ud^*z.
$$
In particular, following the same argument as above, the Fourier inversion in $\tr(g_1)$ and $\tr(g_2)$ variables is given by 
$$
\wh{\RJ}^\rho_{\psi}(a,\xi_1,\xi_2) = 
\int_{\xi_1 z= \xi_2z=1}
\psi(z)|z|^{-2}\ud^*z
$$
which, as a distribution in $(\xi_1,\xi_2)$, is \emph{not} supported on the square class. 

As a result, $\RJ^{\rho}_\psi\neq \RJ^{\rho}_{\psi,\mathrm{Laf}}$. To make it precise, assuming that the construction of Lafforgue works, then after applying the inverse of the Lafforgue transform to $\tr(g_1)$ and $\tr(g_2)$, we would get 
$$
\RJ^{\rho,\p}_{\psi}(\tr(g_1),\tr(g_2)) = 
\int^\pv_{F^\times}
\psi(z+\frac{\tr(g_1)+\tr(g_2)}{z})
\ud^*z.
$$
However, by Theorem \ref{thm:descentheuristic:sl2}, Theorem \ref{thm:descentheuristic:gl2}, and the compatibility between Langlands local gamma factors, for $E_1,E_2$ two étale quadratic algebras of $F$, 
$$
\RJ^{\rho}_{\psi,\mathrm{Ngo}}(\tr(e_1),\tr(e_2))
=
\int^\pv_{F^\times}
\psi(z+\frac{\tr(e_1)+\tr(e_2)}{z})\eta_{E_1}(z)\eta_{E_2}(z)
\ud^*z
$$
which is not the same as $\RJ^{\rho,\p}_{\psi}$. 



\begin{rmk}\label{rmk:exceptionaleg:2}
Although the remedy of Lafforgue fails in general, as we have seen in previous section, it still plays a crucial role in the formulation of the correct kernel function. In a forthcoming work, we will discuss the analogue of Lafforgue transform for $G=\GL_n$.
\end{rmk}
